A Direct Translation from Abstract Cyclic Proofs to Inductive Proofs

We identify the notion of a `well-organized' cyclic proof, show that any cyclic proof can be unfolded to a well-organized one, and present a constructive and relatively simple translation from well-organized cyclic proofs to ordinary well-founded proofs. We work with a general class of cyclic proof systems, and translate from such a system to an induced inductive proof system: a multi-sorted predicate logic that extends the cyclic system with a well-founded induction principle. This setting is broad enough to cover trace-based cyclic proofs and size-change terminating functions. Our unfolding technique is a refinement of earlier annotation-based approaches, and allows us to handle cyclic proofs where the underlying inductive sorts need not be linearly ordered.

==> macros.tex <==
%%novalidate


\usepackage{bbold,isomath}

\makeatletter

%\usepackage[backgroundcolor = lightblue, linecolor = lightblue, bordercolor = lightblue]{todonotes}

% colors
\newcommand\dimm[1]{\textcolor{gray}{{}#1{}}}
\newcommand\alert[1]{\textcolor{red}{{}#1{}}}
\newcommand\highlight[1]{\colorbox{lightgray!50}{\(#1\)}}
\definecolor{lightred}   {HTML}{ee9999}
\definecolor{lightgreen} {HTML}{aaddaa}
\definecolor{lightblue}  {HTML}{9999ee}
\definecolor{lightyellow}{HTML}{ddddaa}
\definecolor{lightpink}  {HTML}{ddaadd}
\definecolor{lightmizu}  {HTML}{aadddd}
\definecolor{gray}       {HTML}{aaaaaa}
\definecolor{lightgray}  {HTML}{dddddd}
\definecolor{darkgray}   {HTML}{222222}

% logic
\newcommand\liff\leftrightarrow
\newcommand\biglor\bigvee
\newcommand\bigland\bigwedge
\providecommand\eqdef{\overset{\smash{\scriptscriptstyle\sf{def}}}=}
\newcommand\defeq\eqdef
\providecommand\colonequiv{\vcentcolon\mspace{-1.2mu}\equiv}
\providecommand\equivcolon{\equiv\mspace{-1.2mu}\vcentcolon}

% brackets
\newcommand\<\langle
\renewcommand\>\rangle
\newcommand\llb\llbracket
\newcommand\rrb\rrbracket

% fonts
\newcommand\bb\mathbb
\providecommand\cal{}
\renewcommand\cal\mathcal
\renewcommand\sf\mathsf
\renewcommand\rm{\relax\ifmmode\expandafter\mathrm\else\expandafter\rmfamily\fi} % llncs uses \rm in text mode
\renewcommand\frak\mathfrak

% category theory
\newcommand\id{\sf{id}}
\newcommand\Mor{\sf{Mor}}
\newcommand\Hom{\sf{Hom}}
\newcommand\End{\sf{End}}
\newcommand\Iso{\sf{Iso}}
\newcommand\Aut{\sf{Aut}}
\newcommand\dom{\sf{dom}}
\newcommand\codom{\sf{codom}}
\newcommand\rng{\sf{rng}}
\renewcommand\mod{\sf{mod}}

% type theory
\newcommand\weak\triangledown
\newcommand\ctx{~\sf{ctx}}
\newcommand\Ctx{\sf{Ctx}}
\newcommand\type{~\sf{type}}
\newcommand\Type{\sf{Type}}
\newcommand\tel{~\sf{tel}}
\newcommand\Tel{\sf{Tel}}
\newcommand\prop{~\sf{prop}}
\newcommand\Prop{\sf{Prop}}
\newcommand\set{~\sf{set}}
\newcommand\Set{\sf{Set}}
\newcommand\refl{\sf{refl}}
\newcommand\app{\sf{app}}
\newcommand\suc{\sf{suc}}
\newcommand\rec{\sf{rec}}
\newcommand\ind{\sf{ind}}
\newcommand\stind{{<}\text-\sf{ind}}
\newcommand\below{\sf{below}}
\newcommand\match{\sf{match}}
\newcommand\Id{\sf{Id}}
\newcommand\W{\rm W}
\newcommand\M{{\makesize{\rm M}{\rm W}}}
\newcommand\Ind{\sf{Ind}}
\newcommand\Coind{\sf{Coind}}
\newcommand\cons{\sf{cons}}
\newcommand\des{\sf{des}}
\providecommand\smt{\mathrel{\ooalign{\(<\)\cr\(-\)}}}
\providecommand\lat{\mathrel{\ooalign{\(>\)\cr\(-\)}}}
\providecommand\smte{\mathrel{\ooalign{\raisebox{1.5pt}{\(\smt\)}\cr\raisebox{-2.5pt}{\(-\)}}}}
\providecommand\late{\mathrel{\ooalign{\raisebox{1.5pt}{\(\lat\)}\cr\raisebox{-2.5pt}{\(-\)}}}}
\newcommand\defl\smt
\newcommand\defle\smte
\newcommand\defg\lat
\newcommand\defge\late
\newcommand\vdasha{\vdash_{\mathrlap{\hspace{-4pt}\scriptscriptstyle\sf A}}}
\newcommand\vdashi{\vdash_{\mathrlap{\hspace{-3.5pt}\scriptscriptstyle\sf I}}}
\newcommand\vdashe{\vdash_{\mathrlap{\hspace{-4pt}\scriptscriptstyle\sf E}}}

% arrows
\providecommand\from\leftarrow
\providecommand\To\Rightarrow
\providecommand\From\Leftarrow
\providecommand\longto\longrightarrow
\providecommand\longfrom\longleftarrow
\providecommand\limplies\rightarrow
\providecommand\limpliedby\leftarrow
\providecommand\leftsquigarrow{\mathrel{\mathpalette\reflect@squig\relax}}
\newcommand{\reflect@squig}[2]{\reflectbox{$\m@th#1\rightsquigarrow$}}
\newcommand\tos       {\mathrel{\to\hspace{-4.25pt}\clipbox{{.65\width} {-\height} 0pt {-\height}}{$\m@th\rightarrow$}}}
\newcommand\toss      {\mathrel{\tos\hspace{-4.25pt}\clipbox{{.65\width} {-\height} 0pt {-\height}}{$\m@th\rightarrow$}}}
\newcommand\disp      {\mathrel{\hspace{-0.175pt}-\raisebox{0.8pt}{\(\scriptstyle\hspace{-1.2pt}\triangleright\)}}}
\newcommand\fib       {\mathrel{\hspace{-0.175pt}-\raisebox{0.8pt}{\(\scriptstyle\hspace{-1.2pt}\triangleright\hspace{-0.8pt}\triangleright\)}}}
\newcommand\tdisp     {\mathrel{\smash{\ooalign{\raisebox{3pt}{\(\scriptstyle\sim\)}\cr\(\disp\)}}}}
\newcommand\tfib      {\mathrel{\smash{\ooalign{\raisebox{3pt}{\(\scriptstyle\sim\)}\cr\(\fib\)}}}}
\newcommand\simeqto   {\mathrel{\smash{\ooalign{\raisebox{3pt}{\(\scriptstyle\sim\)}\cr\(\to\)}}}}
\newcommand\congto    {\mathrel{\smash{\ooalign{\raisebox{3pt}{\(\scriptstyle\sim\)}\cr\(\to\)\cr\raisebox{-2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}}}}}
\newcommand\eqto      {\mathrel{\smash{\ooalign{\(\to\)\cr\raisebox{-2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}}}}}
\newcommand\equivto   {\mathrel{\smash{\ooalign{\raisebox{2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}\cr\(\to\)\cr\raisebox{-2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}}}}}
\newcommand\equivparto{\mathrel{\smash{\ooalign{\hspace{-0.175pt}\(-\)\cr\(\rightrightarrows\)}}}}
\newcommand\equivtos  {\mathrel{\smash{\ooalign{\raisebox{2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}\cr\(\tos\)\cr\raisebox{-2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}}}}}
\newcommand\equivtoss {\mathrel{\smash{\ooalign{\raisebox{2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}\cr\(\toss\)\cr\raisebox{-2pt}{\hspace{-0.175pt}\scalebox{0.85}[1]{\(-\)}}}}}}

\newcommand*\Relbarfill@{\arrowfill@\Relbar\Relbar\Relbar}
\newcommand*\xeq[2][]{\ext@arrow 0055\Relbarfill@{#1}{#2}}

% arrows in tikzcd
\usetikzlibrary{tikzmark}
\usetikzlibrary{cd}
\usetikzlibrary{nfold}
\tikzcdset{pullback/.style = {"\lrcorner"{anchor = center, pos = 0.125}, draw = none}}
\tikzcdset{   equal/.style = {Rightarrow, scaling nfold=2, no head}}
\tikzcdset{   equiv/.style = {Rightarrow, scaling nfold=3, no head}}
\tikzcdset{    disp/.style = {-{Triangle[open]}}}
\tikzcdset{     fib/.style = {-{Triangle[open].Triangle[open]}}}
\tikzcdset{   simeq/.style = {"\raisebox{3pt}      {\(\scriptstyle\sim\)}" {sloped, marking}}, no head}
\tikzcdset{  simeq'/.style = {"\raisebox{-1.5pt}   {\(\scriptstyle\sim\)}" {sloped, marking}}, no head}
\tikzcdset{   simeq/.style = {"\raisebox{3pt}      {\(\scriptstyle\sim\)}" {sloped, marking}}}
\tikzcdset{  simeq'/.style = {"\raisebox{-1.5pt}   {\(\scriptstyle\sim\)}" {sloped, marking}}}
\tikzcdset{    iden/.style = {"\raisebox{-2pt}{\scalebox{0.85}[1]{\(-\)}}" {sloped, marking}}}
\tikzcdset{   iden'/.style = {"\raisebox{2pt} {\scalebox{0.85}[1]{\(-\)}}" {sloped, marking}}}
\tikzcdset{    tfib/.style = {simeq,  fib}}
\tikzcdset{   tfib'/.style = {simeq', fib}}
\tikzcdset{     iso/.style = {simeq,  iden}}
\tikzcdset{    iso'/.style = {simeq', iden'}}

\prfinterspace = 2em

% colored accents
\def\coloredaccent#1#2#3{% #1=color, #2=accent, #3=nucleus
   \colorlet{outcolor}{.}
   \textcolor{#1}{#2{\textcolor{outcolor}{#3}}}
}

% set stmry bold fonts to the normal ones to silence warnings
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}

% a version of \prftree where the assumptions are stacked and left aligned
\newcommand\prfstack{\prf@init\prf@Nstack}
% read in the options
\newcommand\prf@Nstack{\@ifnextchar[{\prf@stackoptions}{\prf@stackrule}}
\def\prf@stackoptions[#1]{\prf@opts#1,]\prf@Nstack}
% if there is no rule add an empty one
\def\prf@stackrule{%
    \edef\prf@rulechoice{\ifprf@rule\else{}\fi}%
    \expandafter\prf@stacklabel\prf@rulechoice%
}
% if there is no label add an empty one
\def\prf@stacklabel#1{%
    \def\prf@hackpar{#1}%
    \edef\prf@labelchoice{{\noexpand\prf@hackpar}\ifprf@label\else{}\fi}%
    \expandafter\prf@stackinit\prf@labelchoice%
}
% do the initiation and call the recursive macro
\newcommand\prf@stackinit[3]{%
    \ifprf@label\raisebox{0.46\baselineskip}{\text{#2}}\hspace*\prflabelskip\fi%
    \begin{array}[b]{@{}l@{}l@{}}%
    \hspace*\prflineextra%
    \@ifnextchar\bgroup%
        {\prf@stackrec{#1}{#2}{#3}}%
        {\prf@stackrec{#1}{#2}{}{#3}}%
}
% add newlines after arguments and do the finalisation
\newcommand\prf@stackrec[4]{\@ifnextchar\bgroup%
    {\prf@stackrec{#1}{#2}{%
        #3%
        \ifprfSTRUToption\mathstrut\fi%
        \hspace*\prflineextra\\%
        \hspace*\prflineextra% 
        #4%
        %
    }}{%
        #3%
        \ifprfSTRUToption\mathstrut\fi%
        \hspace*\prflineextra\\%
        \noalign{\hrule height\prflinethickness\vspace*\prflinepadafter}%
        \hspace*\prflineextra%
        #4%
        \hspace*\prflineextra%
        \end{array}%
        \ifprf@rule\hspace*\prfrulenameskip\raisebox{0.46\baselineskip}{\text{#1}}\fi%
    }%
}

% blackboard bold logical symbols
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
    <5> <6> <7> <8> <9> <10> gen * matha
    <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
}{}
\newcommand\bbbot{\rotatebox[origin=c]{180}{\(\bbtop\)}}
\newcommand\bbtop{\ooalign{\makesize{\rotatebox[origin=c]{90}{\(-\)}\hspace{-1.25ex}\rotatebox[origin=c]{90}{\(-\)}}{\(-\)}\cr\raisebox{3pt}{\(-\)}}}
\newcommand\bblor{\mathbin{\raisebox{.1ex}{\rotatebox[origin=c]{90}{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}}}}
\newcommand\bbland{\mathbin{\raisebox{.1ex}{\rotatebox[origin=c]{-90}{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}}}}
\newcommand\bbto\To
\newcommand\bbmapsto\Mapsto
\newcommand\bbforall{\rotatebox[origin=c]{180}{\reflectbox{\(\bb A\)}}}
\newcommand\bbexists{\rotatebox[origin=c]{180}{\(\bb E\)}}
\newcommand\bbplus{\mathbin{\ooalign{\makesize{\rotatebox[origin=c]{90}{\(-\)}\hspace{-1.25ex}\rotatebox[origin=c]{90}{\(-\)}}{\(-\)}\cr\(-\)}}}
\newcommand\bbtimes{\mathbin{\rotatebox[origin=c]{45}{\(\bbplus\)}}}
\newcommand\bbeq\equiv
\newcommand\bbl{\mathbin{\ooalign{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}}}
\newcommand\bble{\mathbin{\smash{\ooalign{\raisebox{1.5pt}{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}\cr\raisebox{-3pt}{\(-\)}}}}}
\newcommand\bbg{\mathbin{\rotatebox[origin=c]{180}{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}}}
\newcommand\bbge{\mathbin{\smash{\ooalign{\raisebox{1.5pt}{\rotatebox[origin=c]{180}{\usefont{U}{matha}{m}{n}\symbol{\string"CE}}}\cr\raisebox{-3pt}{\(-\)}}}}}
\providecommand\smt{\mathrel{\ooalign{\(<\)\cr\(-\)}}}
\providecommand\lat{\mathrel{\ooalign{\(>\)\cr\(-\)}}}
\providecommand\smte{\mathrel{\ooalign{\raisebox{1.5pt}{\(\smt\)}\cr\raisebox{-2.5pt}{\(-\)}}}}
\providecommand\late{\mathrel{\ooalign{\raisebox{1.5pt}{\(\lat\)}\cr\raisebox{-2.5pt}{\(-\)}}}}
\providecommand\Subseteq{\mathrel{\ooalign{\raisebox{1.5pt}{\(\Subset\)}\cr\raisebox{-4pt}{\(-\)}}}}
\providecommand\Supseteq{\mathrel{\ooalign{\raisebox{1.5pt}{\(\Supset\)}\cr\raisebox{-4pt}{\(-\)}}}}

% improves the vertical space of vdots
\renewcommand\vdots{\vbox{\baselineskip4\p@ \lineskiplimit\z@ \hbox{.}\hbox{.}\hbox{.}}}

% resizes the first argument to the size of the second argument
\newskip\makesize@widthfrom
\newskip\makesize@widthto
\newskip\makesize@widthhalfdiff
\newcommand\makesize[3][c]{%
    \ifmmode%
        \text{\makesize@do{#1}{\(\m@th{#2}\)}{\(\m@th{#3}\)}}%
    \else%
        \makesize@do{#1}{#2}{#3}%
    \fi%
}
\newcommand\makesize@do[3]{%
    \settowidth\makesize@widthfrom{#2}%
    \settowidth\makesize@widthto{#3}%
    \setlength\makesize@widthhalfdiff{0.5\makesize@widthto - 0.5\makesize@widthfrom}%
    %
    \if#1s%
        \makebox[\makesize@widthto][s]{#2}%
    \else%
        \vphantom{#3}%
        %
        \if#1l\smash{#2}\fi%
        \hspace*{\makesize@widthhalfdiff}%
        \if#1c\smash{#2}\fi%
        \hspace*{\makesize@widthhalfdiff}%
        \if#1r\smash{#2}\fi%
    \fi%
}

% a gathering of inference rules in a full-width frame, named in its top-left
% corner; the frame breaks across pages
\mdfdefinestyle{rulesframe}{%
    % same weight as the proof lines of the rules inside
    linewidth=\prflinethickness,
    % a block splits only as a last resort: the penalty between rows (set in the
    % environment) makes any other break cheaper, and mdframed itself ejects the
    % page rather than split when fewer than two baselines are left
    nobreak=false,
    splittopskip=6pt,
    splitbottomskip=6pt,
    % draws the two edges at a division, which are dashed below
    everyline=true,
    % the frame is exactly the text block, flush left and right. Widening it to
    % preserve the measure is not worth it: mdframed hangs the extra width off
    % the right (align=center pads with \fill inside a makebox that still starts
    % at the left margin, and leftmargin is then ignored).
    linecolor=darkgray,
    innertopmargin=6pt,
    innerbottommargin=6pt,
    innerleftmargin=6pt,
    innerrightmargin=6pt,
    % rigid, so that a page containing unbreakable blocks stretches its other
    % glue rather than blowing up the gap around a block
    skipbelow=10pt,
    % otherwise the contents open with a \vspace*{-\parskip}, which shifts them
    % by an amount that depends on the class; the environment sets \parskip to
    % zero inside instead, so the contents start exactly innertopmargin down
    suppressfirstparskip=false,
}
% An edge at a division is dashed, so that a frame stopping mid-page reads as
% continuing overleaf rather than as a block that happens to end there. mdframed
% draws these two edges only under everyline, and the four edges of an undivided
% block go through the @single macros, so redefining the split ones is enough.
\newlength\rules@dashlength
\newlength\rules@dashgap
\setlength\rules@dashlength{3pt}
\setlength\rules@dashgap{3pt}
\newlength\rules@dima
\newlength\rules@dimb
\newlength\rules@dimc
% takes the raise, width and thickness that the solid \rule would have had, and
% matches its dimensions: an hbox of vrules raised into the same position
\newcommand\rules@dashrule[3]{%
    \setlength\rules@dima{#1}%
    \setlength\rules@dimb{#2}%
    \setlength\rules@dimc{#3}%
    \raisebox\rules@dima{%
        \hb@xt@\rules@dimb{%
            \xleaders\hbox{\vrule\@width\rules@dashlength
                                 \@height\rules@dimc\@depth\z@
                           \hskip\rules@dashgap}\hfil}}%
}
% the vertical rules sit outside the bounding box, so a horizontal edge spans
% the box plus whichever of them is drawn
\def\rules@edgewidth{%
    \dimexpr\mdfboundingboxtotalwidth
        \ifbool{mdf@rightline}{+\mdf@middlelinewidth@length}{}%
        \ifbool{mdf@leftline}{+\mdf@middlelinewidth@length}{}\relax}
\def\rules@dashedbottom{%
    \rlap{%
        \ifbool{mdf@leftline}{\hspace*{-\mdf@middlelinewidth@length}}{}%
        \mdf@linecolor@default
        \ifbool{mdf@bottomline}%
            {\rules@dashrule
                {\dimexpr-\mdfboundingboxdepth-\mdf@middlelinewidth@length\relax}%
                {\rules@edgewidth}{\mdf@middlelinewidth@length}}{}%
    }%
}
\newcommand\rules@dashedtop[1]{%
    \rlap{%
        \ifbool{mdf@leftline}{\hspace*{-\mdf@middlelinewidth@length}}{}%
        \mdf@linecolor@default
        \ifbool{mdf@topline}%
            {\rules@dashrule{#1}{\rules@edgewidth}{\mdf@middlelinewidth@length}}{}%
    }%
}
\let\mdf@frame@bottomline@first\rules@dashedbottom
\let\mdf@frame@bottomline@middle\rules@dashedbottom
\def\mdf@frame@topline@second{%
    \rules@dashedtop{\dimexpr\mdfboundingboxheight-\mdfboundingboxdepth
                             +\mdf@innerbottommargin@length\relax}}
\def\mdf@frame@topline@middle{%
    \rules@dashedtop{\dimexpr\mdfboundingboxtotalheight-\mdfboundingboxdepth\relax}}
% A part continuing overleaf has no top margin: mdframed only puts splittopskip
% above it, which is measured to the first baseline and so vanishes under a row
% of rules taller than it. The pad restores the margin, and is taken off the
% page height that mdframed fills, so the padded part still fits. It is zero
% outside the environment, leaving any other mdframed untouched.
\newlength\rules@splitpad
\newcommand\rules@patchfailed{%
    \PackageWarning{rules}{mdframed has changed; continued parts lose their
                           top margin}}
\newcommand\rules@padtop[1]{%
    \ifvoid#1\else
        \setbox#1\vbox{\kern\rules@splitpad\unvbox#1}%
    \fi
}
\pretocmd\mdf@putbox@second{\rules@padtop\mdf@splitbox@one}{}{\rules@patchfailed}
\pretocmd\mdf@putbox@middle{\rules@padtop\mdf@splitbox@two}{}{\rules@patchfailed}
\patchcmd\mdf@put@frame@ii
    {\setlength{\mdf@freevspace@length}{\vsize}}
    {\setlength{\mdf@freevspace@length}{\dimexpr\vsize-\rules@splitpad\relax}}
    {}{\rules@patchfailed}

% Consecutive blocks share an edge: the flag records that the last thing set was
% a block, and any paragraph of text in between clears it again. When it is set,
% the skip above cancels the previous block's skip below and overlaps the two
% rules, so a run of blocks reads as one framed column.
\newif\ifrules@prev
\newlength\rules@above
% how much of the page a block has to be able to fill before it is worth
% dividing. With less than this free, the page ends here and the block starts
% whole overleaf; with more, mdframed splits it rather than strand the space
\newlength\rules@minsplit
\setlength\rules@minsplit{0.25\textheight}
\AddToHook{para/begin}{\global\rules@prevfalse}
% The name is set as the line opening the contents, rather than as an mdframed
% frametitle, whose position depends on \parskip and on how the title box is
% stacked. Its box is raised and pulled right by the margin and rule width that
% mdframed has just set, so its top and right edges lie on the frame's rules
% whatever their values. The line has no height but keeps the box's depth, so
% the rules start below the box. Being part of the contents, it appears on the
% first part of a divided block only.
\newsavebox\rules@namebox
\newcommand\rules@name[1]{%
    % ruled in the frame's colour, so that the edges it shares with the frame
    % are seamless
    \sbox\rules@namebox{\setlength\fboxrule{\mdf@middlelinewidth@length}%
                        \mdf@linecolor@default
                        \fbox{\normalcolor\normalfont\scshape#1}}%
    \nointerlineskip
    \hb@xt@\hsize{\hfil
        \raisebox{\dimexpr\mdf@innertopmargin@length+\mdf@middlelinewidth@length
                          -\ht\rules@namebox\relax}[\z@]%
                 {\usebox\rules@namebox}%
        \kern-\dimexpr\mdf@innerrightmargin@length
                      +\mdf@middlelinewidth@length\relax}%
    \nobreak\nointerlineskip
}
\newenvironment{rules}[1]{%
    \ifrules@prev
        \setlength\rules@above{-10pt}%
        \addtolength\rules@above{-\prflinethickness}%
    \else
        \setlength\rules@above{10pt}%
    \fi
    \par\needspace{\rules@minsplit}%
    \setlength\rules@splitpad{6pt}%
    \mdframed[style=rulesframe,skipabove=\rules@above]%
    \parskip\z@skip
    \rules@name{#1}%
    \abovedisplayskip=\z@ \abovedisplayshortskip=\z@
    \belowdisplayskip=\z@ \belowdisplayshortskip=\z@
    % gather* is unbreakable by default, which leaves mdframed no legal point to
    % split at. Level 1 lowers the penalty between rows to 9999: still finite, so
    % a tall block can be divided rather than pushed whole onto the next page and
    % leaving this one half empty, but dear enough that nothing else splits.
    \allowdisplaybreaks[1]%
    \csname gather*\endcsname
}{%
    \csname endgather*\endcsname
    \endmdframed
    \global\rules@prevtrue
}

\makeatother
